Predictive Runtime Monitoring for Mobile Robots using Logic-Based Bayesian Intent Inference

We propose a predictive runtime monitoring framework that forecasts the distribution of future positions of mobile robots in order to detect and avoid impending property violations such as collisions with obstacles or other agents. Our approach uses a restricted class of temporal logic formulas to represent the likely intentions of the agents along with a combination of temporal logic-based optimal cost path planning and Bayesian inference to compute the probability of these intents given the current trajectory of the robot. First, we construct a large but finite hypothesis space of possible intents represented as temporal logic formulas whose atomic propositions are derived from a detailed map of the robot's workspace. Next, our approach uses real-time observations of the robot's position to update a distribution over temporal logic formulae that represent its likely intent. This is performed by using a combination of optimal cost path planning and a Boltzmann noisy rationality model. In this manner, we construct a Bayesian approach to evaluating the posterior probability of various hypotheses given the observed states and actions of the robot. Finally, we predict the future position of the robot by drawing posterior predictive samples using a Monte-Carlo method. We evaluate our framework using two different trajectory datasets that contain multiple scenarios implementing various tasks. The results show that our method can predict future positions precisely and efficiently, so that the computation time for generating a prediction is a tiny fraction of the overall time horizon.

==> predictive_rv.tex <==





Using the Bayesian intent inference framework, we can compute the probability distribution over hypotheses. However, the aforementioned approach is often not appropriate to be implemented in real time because constructing the required number of product automata is computationally expensive if we have a long list of hypotheses. Two approaches exist to relax this problem: (1) increasing the average size of cells of a FTS or (2) reducing the number of product automata.

\textbf{Adjusting Cell Size of FTS}. The minimum time required in real time operation depends on the size of cells. If it takes $T$ seconds for a robot to traverse from one cell to another, our framework should finish all required computations in $t<<T$ to ensure that we can exploit the output of the framework. In other words, if the framework requires $t$ seconds for computations, we can adjust the size of cells so that the robot needs at least $T$ seconds before moving to other cells. There are some cases where this approach benefits.

For instance, if we are trying to predict the future position of an unmanned aerial vehicle (UAV), we may not be interested in future positions in $1$-$2$ seconds. Instead, we may want to see where the UAV is going in the long run. In this case, using a large map with large size of cells is enough or more effective. 

\textbf{Constructing Only One Product Automaton}. In this paper, we will focus on the second approach. Considering the most of missions for mobile robots are \emph{safety} (avoidance) and \emph{reachability} (coverage), we need only one product automaton to handle those two requirements, i.e., $\lozenge \pi$ and $\square \neg \pi$. Before we introduce this automaton, we will present a directed acyclic graph (DAG) to explain the idea of this approach.

Assume that we have a FTS that contains $N$ cells and $K$ regions of interest. First, we make a DAG with one vertex representing “visit nothing”, $\square \neg \pi_0 \wedge \square \neg \pi_1 \wedge \cdots \wedge \square \neg \pi_K$. This first vertex is our first hypothesis. Next, we assume that a robot visits one of regions while avoiding the rest, for example, “visit $\pi_0$ while avoiding others”, $\lozenge \pi_0 \wedge \square \neg \pi_1 \wedge \cdots \wedge \square \neg \pi_K$. To represent this hypotheses, we add $K$ vertices to the DAG connecting them to the root vertex using edges. As a result, we have the $K+1$ hypothesis (avoid all or visit one of $K$). In this manner, we can add more vertices under each vertex in the graph until requirements turn into “visit all regions”. After finishing this construction, we will have a DAG which has $2^K$ nodes representing all possible combinations of $\lozenge \pi_{1 \cdots K}$ and $\square \neg \pi_{1 \cdots K}$. Fig.~\ref{fig:one_automaton} shows the example of a DAG when we have three regions of interest. 

\begin{figure}[t]
\begin{tikzpicture}
\node (n0) at (0,0) {\includegraphics[width=0.48\textwidth]{figures/one_automaton.png}};
\end{tikzpicture}
\caption{TODO:example of one automaton and DAG. They are the same}\label{fig:one_automaton}
\end{figure}

Here, considering the DAG includes all possible routes, we can easily convert this graph to a B{\"u}chi automaton. Like this DAG, the automata of the LTL specification $\lozenge \pi_0 \wedge \lozenge \pi_1 \lozenge \cdots \wedge \lozenge \pi_K$ has all possible paths for visiting all $K$ regions as shown in fig.~\ref{fig:one_automaton}. We assume that all regions of interest do not have intersections adding some specifications to avoid unnecessary edges in the automaton. Therefore, the final specification is $\square \neg (\pi_0 \wedge \pi_1) \wedge \square \neg (\pi_0 \wedge \pi_2) \wedge \cdots \wedge \square \neg (\pi_{K-1} \wedge \pi_K) \wedge \lozenge \pi_0 \wedge \lozenge \pi_1 \lozenge \cdots \wedge \lozenge \pi_N$. In this automaton, if we consider each node as our hypothesis, we can check $2^K$ hypothesis by changing the accepting state in the automaton. For example, we can set the initial state into the initial and accepting state for the first hypothesis, “visit nothing”. Likewise, we can reset the accepting state to another state to represent different hypothesis. Using this approach, we can reduce the number of computations from $2^K$ to 1 since we only build one product.

\subsection{Monte Carlo Simulation}
Once we finish inferring intents of a robot, we can solve the \emph{predictive monitoring problem}. In addition to predicting position $\mathbf{x}_{t+h}$ at the current time $t$, we are able to compute the probability of reaching at $\mathbf{x}_{t+h}$ using the posterior distribution over hypothesis and Eq.~\ref{eq:boltzmann}. However, the analytic solution is computationally expensive to be implemented in real time. Instead, we use the Monte-Carlo method to predict future positions and corresponding probability. Given prediction horizon $h$, the prediction procedure is as follows:
\begin{compactenum}
\item At time $t$, We sample one intent from the posterior distribution.
\item Starting from the current position, we can compute the probability distribution of all neighboring states using Eq.~\ref{eq:boltzmann} given the intent.
\item Next, we draw one of neighboring states from the probability distribution. 
\item From the state drawn above (new current position at time $t+1$), repeat 2)-3) to find next states until $t+h$.
\item Repeat 1)-4) to sample more predicted positions.
\item Based on the predicted position, compute the probability of reaching each cell.
\end{compactenum}

In this paper, we run 300 Monte-Carlo simulations for prediction and obtain the probability distribution of future positions. 

